Spatial Object Recommendation with Hints: When Spatial Granularity Matters

Existing spatial object recommendation algorithms generally treat objects identically when ranking them. However, spatial objects often cover different levels of spatial granularity and thereby are heterogeneous. For example, one user may prefer to be recommended a region (say Manhattan), while another user might prefer a venue (say a restaurant). Even for the same user, preferences can change at different stages of data exploration. In this paper, we study how to support top-k spatial object recommendations at varying levels of spatial granularity, enabling spatial objects at varying granularity, such as a city, suburb, or building, as a Point of Interest (POI). To solve this problem, we propose the use of a POI tree, which captures spatial containment relationships between POIs. We design a novel multi-task learning model called MPR (short for Multi-level POI Recommendation), where each task aims to return the top-k POIs at a certain spatial granularity level. Each task consists of two subtasks: (i) attribute-based representation learning; (ii) interaction-based representation learning. The first subtask learns the feature representations for both users and POIs, capturing attributes directly from their profiles. The second subtask incorporates user-POI interactions into the model. Additionally, MPR can provide insights into why certain recommendations are being made to a user based on three types of hints: user-aspect, POI-aspect, and interaction-aspect. We empirically validate our approach using two real-life datasets, and show promising performance improvements over several state-of-the-art methods.

==> alg-train.tex <==
\setlength{\algomargin}{0.5em} 
\setlength{\textfloatsep}{0.1cm}
\begin{algorithm}[t]
	\small
	\caption{\small The Training Algorithm }   
	\label{alg-train}   
	\begin{algorithmic}[1] %"1" represents that it will show number in each row  
		\REQUIRE  %Input  
		a user set \userSet, a POI set \poiSet, user-POI interaction data \interactionSet, a POI tree \poiTree, the number of interation \numIter, the batch size \batchSize
		\ENSURE all the model paramters $\Theta$
		%\STATE Initialize parameters xxx
		\STATE $nBatch$ = $|\interactionSet| / \batchSize$
		\STATE $iter$ = $0$
		\WHILE {$iter \textless \numIter$} 											
		\STATE Shuffle(\interactionSet)
		\FOR {$bId=0; bId \textless nBatch; bId$++}		
		\STATE $\interactionSet_{b}$  = ExtractBatchData($bId$, \interactionSet)	
		\STATE Get the POI set $\poiSet_{b}$ occurred in $\interactionSet_{b}$
		\STATE Divide $\poiSet_{b}$ into a positive POI set \{$\poiSet_{b}^{1+},\poiSet_{b}^{2+},...,\poiSet_{b}^{\poiTreeNum+}$\} based on the tree structure \poiTree
		\STATE Sample a negative POI set \{$\poiSet_{b}^{1-},\poiSet_{b}^{2-},...,\poiSet_{b}^{\poiTreeNum-}$\} correspondingly
		\STATE Take a gradient step to optimize Eq. \ref{equ-loss}
		\ENDFOR 																			
		\ENDWHILE						
	\end{algorithmic} 
\end{algorithm}








==> fig-exp1.tex <==
%%%%%% H_1 level
\begin{figure}[t]
	\centering
	\subfloat[\textit{Beijing}]{
		\label{fig:Precision:one}
		\includegraphics[width=\graphscale\textwidth]{figure/result/aoi_Precision.pdf}
	}
	\subfloat[\textit{Chengdu}]{
		\label{fig:Precision_chengdu:one}
		\includegraphics[width=\graphscale\textwidth]{figure/result/aoi_Precision_chengdu.pdf}
	}
	\vspace{-2ex}
	\subfloat[\textit{Beijing}]{
		\label{fig:Recall:one}
		\includegraphics[width=\graphscale\textwidth]{figure/result/aoi_Recall.pdf}
	}
	\subfloat[\textit{Chengdu}]{
		\label{fig:Recall_chengdu:one}
		\includegraphics[width=\graphscale\textwidth]{figure/result/aoi_Recall_chengdu.pdf}
	}
	\vspace{-2ex}
	\subfloat[\textit{Beijing}]{
		\label{fig:NDCG:one}
		\includegraphics[width=\graphscale\textwidth]{figure/result/aoi_NDCG.pdf}
	}
	\subfloat[\textit{Chengdu}]{
		\label{fig:NDCG_chengdu:one}
		\includegraphics[width=\graphscale\textwidth]{figure/result/aoi_NDCG_chengdu.pdf}
	}
	\vspace{-2ex}
	\caption{Performance Comparison of Methods on \poiTreeLayerOne level.}
	\label{fig:results:one}
	\vspace{-4ex}
\end{figure}


%%%%%% H_2 level
\begin{figure}[t]
	\centering
	\subfloat[\textit{Beijing}]{
		\label{fig:Precision:two}
		\includegraphics[width=\graphscale\textwidth]{figure/result/parent_Precision.pdf}
	}
	\subfloat[\textit{Chengdu}]{
		\label{fig:Precision_chengdu:two}
		\includegraphics[width=\graphscale\textwidth]{figure/result/parent_Precision_chengdu.pdf}
	}
	\vspace{-2ex}
	\subfloat[\textit{Beijing}]{
		\label{fig:Recall:two}
		\includegraphics[width=\graphscale\textwidth]{figure/result/parent_Recall.pdf}
	}
	\subfloat[\textit{Chengdu}]{
		\label{fig:Recall_chengdu:two}
		\includegraphics[width=\graphscale\textwidth]{figure/result/parent_Recall_chengdu.pdf}
	}
	\vspace{-2ex}
	\subfloat[\textit{Beijing}]{
		\label{fig:NDCG:two}
		\includegraphics[width=\graphscale\textwidth]{figure/result/parent_NDCG.pdf}
	}
	\subfloat[\textit{Chengdu}]{
		\label{fig:NDCG_chengdu:two}
		\includegraphics[width=\graphscale\textwidth]{figure/result/parent_NDCG_chengdu.pdf}
	}
	\vspace{-2ex}
	\caption{Performance Comparison of Methods on \poiTreeLayerTwo level.}
	\label{fig:results:two}
	\vspace{-5ex}
\end{figure}



























\iffalse
\begin{figure*}
	\begin{subfigure}[b]{0.167\textwidth}
		\includegraphics[width=\textwidth]{example_a}
		\vspace{-2em}
		\caption{}
		\label{fig:example_a}
	\end{subfigure}
	\begin{subfigure}[b]{0.167\textwidth}
		\includegraphics[width=\textwidth]{example_b}
		\vspace{-2em}
		\caption{}
		\label{fig:example_b}
	\end{subfigure}
	\begin{subfigure}[b]{0.251\textwidth}
		\includegraphics[width=\textwidth]{example_c}
		\vspace{-2em}
		\caption{}
		\label{fig:example_d}
	\end{subfigure}
	\begin{subfigure}[b]{0.204\textwidth}
		\includegraphics[width=\textwidth]{example_d}
		\vspace{-2em}
		\caption{}
		\label{fig:example_e}
	\end{subfigure}
	\begin{subfigure}[b]{0.167\textwidth}
		\includegraphics[width=\textwidth]{example_e}
		\vspace{-2em}
		\caption{}
		\label{fig:example_f}
	\end{subfigure}
	\vspace{-1em}
	\caption{An example of HashICM processing.(a)Event-related hashtag graph construction using pair-wise hashtag correlation;(b)Edge pruning by similarity;(c)Setting the probability for each neighbour of seed h1 by finding the topic distribution of h1 with the maximum probability;(d)Activating neighbours of h1;(e)h2 is activated and selected.}
	\label{example}
\end{figure*}
\fi


==> fig-exp11.tex <==
%%%%%% H_3 level
\begin{figure}[t]
	\centering
	\subfloat[\textit{Beijing}]{
		\label{fig:Precision:three}
		\includegraphics[width=\graphscale\textwidth]{figure/result/child_Precision.pdf}
	}
	\subfloat[\textit{Chengdu}]{
		\label{fig:Precision_chengdu:three}
		\includegraphics[width=\graphscale\textwidth]{figure/result/child_Precision_chengdu.pdf}
	}
	\vspace{-2ex}
	\subfloat[\textit{Beijing}]{
		\label{fig:Recall:three}
		\includegraphics[width=\graphscale\textwidth]{figure/result/child_Recall.pdf}
	}
	\subfloat[\textit{Chengdu}]{
		\label{fig:Recall_chengdu:three}
		\includegraphics[width=\graphscale\textwidth]{figure/result/child_Recall_chengdu.pdf}
	}
	\vspace{-2ex}
	\subfloat[\textit{Beijing}]{
		\label{fig:NDCG:three}
		\includegraphics[width=\graphscale\textwidth]{figure/result/child_NDCG.pdf}
	}
	\subfloat[\textit{Chengdu}]{
		\label{fig:NDCG_chengdu:three}
		\includegraphics[width=\graphscale\textwidth]{figure/result/child_NDCG_chengdu.pdf}
	}
	\vspace{-2ex}
	\caption{Performance Comparison of Methods on \poiTreeLayerThree level.}
	\label{fig:results:three}
	\vspace{-5ex}
\end{figure}
